XF2T: Cross-lingual Fact-to-Text Generation for Low-Resource Languages

Multiple business scenarios require an automated generation of descriptive human-readable text from structured input data. Hence, fact-to-text generation systems have been developed for various downstream tasks like generating soccer reports, weather and financial reports, medical reports, person biographies, etc. Unfortunately, previous work on fact-to-text (F2T) generation has focused primarily on English mainly due to the high availability of relevant datasets. Only recently, the problem of cross-lingual fact-to-text (XF2T) was proposed for generation across multiple languages alongwith a dataset, XALIGN for eight languages. However, there has been no rigorous work on the actual XF2T generation problem. We extend XALIGN dataset with annotated data for four more languages: Punjabi, Malayalam, Assamese and Oriya. We conduct an extensive study using popular Transformer-based text generation models on our extended multi-lingual dataset, which we call XALIGNV2. Further, we investigate the performance of different text generation strategies: multiple variations of pretraining, fact-aware embeddings and structure-aware input encoding. Our extensive experiments show that a multi-lingual mT5 model which uses fact-aware embeddings with structure-aware input encoding leads to best results on average across the twelve languages. We make our code, dataset and model publicly available, and hope that this will help advance further research in this critical area.

==> scratch.tex <==
Generating text from structured data is challenging because 
it requires bridging the gap between (i) structure and natural language (NL) and (ii) semantically underspecified input and
fully specified NL output. 

Multilingual generation brings in an additional challenge: that of generating into languages with varied word order and morphological properties. 



In this work,
we focus on Abstract Meaning Representations (AMRs) as structured input, where previous research has overwhelmingly focused on
generating only into English. We leverage advances in cross-lingual embeddings, pretraining, and multilingual models to create multilingual AMR-to-text models that generate in
twenty one different languages. For eighteen
languages, based on automatic metrics, our
multilingual models surpass baselines that generate into a single language. We analyse the
ability of our multilingual models to accurately
capture morphology and word order using human evaluation, and find that native speakers
judge our generations to be fluent.

